Rigorous Error Analysis for Logarithmic Number Systems

Logarithmic Number Systems (LNS) hold considerable promise in helping reduce the number of bits needed to represent a high dynamic range of real-numbers with finite precision, and also efficiently support multiplication and division. However, under LNS, addition and subtraction turn into non-linear functions that must be approximated - typically using precomputed table-based functions. Additionally, multiple layers of error correction are typically needed to improve result accuracy. Unfortunately, previous efforts have not characterized the resulting error bound. We provide the first rigorous analysis of LNS, covering detailed techniques such as co-transformation that are crucial to implementing subtraction with reasonable accuracy. We provide theorems capturing the error due to table interpolations, the finite precision of pre-computed values in the tables, and the error introduced by fix-point multiplications involved in LNS implementations. We empirically validate our analysis using a Python implementation, showing that our analytical bounds are tight, and that our testing campaign generates inputs diverse-enough to almost match (but not exceed) the analytical bounds. We close with discussions on how to adapt our analysis to LNS systems with different bases and also discuss many pragmatic ramifications of our work in the broader arena of scientific computing and machine learning.

==> sections/add-rel-work.tex <==

Maybe add some comparisons with POSIT?

What else?

Also, there are more direct uses of multiplication such as in multiplicative weight-update schemes using ML training such as MADAM~\cite{madam}---again requiring cost-reductions of multiplication.

POSIT also

==> sections/design.tex <==
%In contrast to many existing algorithms' emphasis on prior accessors, our design is inspired by a "safety property" which tracks thread sets that may safely access a particular memory location in the future. Though these viewpoints are equivalent, the high thread counts and hierarchical nature of GPU architectures lend themselves more naturally to reasoning about work groups and scoped operations than complex interactions between individual threads.

We begin walking through the high-level design of \toolname by incrementally developing the intuition behind its internal finite-state-machine (FSM). We then provide implementation details in the following section.

 
\begin{figure}[]
    %\centering
    \includegraphics[width=0.5\textwidth]{figures/ssm_nosync.png}
    \caption{State-Machine for No Synchronization (self loops omitted)}
    \label{fig:ssm_nosync}
\end{figure}


\subsection{High-level idea} % and even higher-level SM

Our design is based around the built-in synchronization primitives available in GPUs (such as \emph{\_\_syncthreads}) as opposed to focusing on the full generality of CPU parallel programming patterns. Our method does not preclude the handling of fine-grained thread synchronization, but we instead focus on optimizing the most common and impactful forms of thread communication in GPUs.

\textbf{The primary motivation of this work is the observation that an arbitrary memory access history may be compactly represented with constant-sized state.}

This is achieved by enumerating equivalence classes of possible thread access histories to a single memory location. For example, if a thread reads the same memory location multiple times, we need not record each access separately. A single thread ID and a flag indicating a read access by that ID suffices.
%
Going a step further, in a program with only 2 threads, if both threads concurrently read the same memory location (in any order and any number of times), it suffices to only track the ID of either accessor along with a flag indicating that {\em multiple} threads have read this location.

In the fully general case, this would require $2^T$ flags to track all possible thread relations between $T$ accessing threads. However, due to the hierarchical and symmetric nature of the shared memory scopes, instead of tracking individual threads at every memory interaction, {\em we only track 
only the hierarchical scope shared by the accessing threads}.
%
These scopes provide naturally symmetric work groups that are uniquely determined by the ID of any thread within the group (i.e., certain bits of a global thread ID). As such, a single identifier (for example, the last accessing thread ID) and a flag representing the scope of access (i.e., thread-block scope) are sufficient to characterize a large class of unbounded access histories (for example, arbitrary reads from multiple threads within the same thread-block).

Motivated by this design, we encapsulate all equivalence classes of read, write, and atomic memory accesses along with the hierarchical synchronization primitives into an explicit state-machine containing 25 unique states.



\subsection{Lower-level details}


Since the complete state-machine is difficult to unambiguously convey in words, we will instead further build the intuition leading to our final state-machine through more concrete examples.

\input{figures/code_rwrace_nosync}

First, consider a CUDA program containing only reads and writes to global memory, with no form of synchronization, such as the code shown in Listing~\ref{lst:rw-nosync}. We claim that the state-machine displayed in Figure~\ref{fig:ssm_nosync}, along with a single prior accessor ID, is sufficient to track any and all data races that may occur in such programs.

To monitor the $data$ array for races, we create a corresponding shadow value for each index, as shown in Figure~\ref{fig:ssm_shadow}.
%
Initially, all shadow values are set to the \textbf{INIT} state, indicating that no memory accesses have occurred.
%
The first access to a tracked memory cell is the read on line 4, at which point some thread(s) will access $shadow[0]$ and find it to be in the \textbf{INIT} state, and attempt to update $shadow[0]$ to store its own thread ID and the new \textbf{READ} state.
%
We only allow one thread to atomically update $shadow[0]$ from the \textbf{INIT} state, while all other accessors will find
the newly updated record and recalculate their new shadow state (all achieved through CUDA atomic primitives).

In this example, since there is no synchronization considered, the only thread scope needed is whether accessors are the (S)ame thread, otherwise the largest shared scope is the (G)lobal scope (i.e. all threads.)
%
Thus, all other concurrent threads executing the read of $data[0]$ will now transition $shadow[0]$'s state; if a thread finds $shadow[0]$ in the \textbf{READ} state, it will attempt to update to \textbf{GLOBAL READ} (as well as store its own thread ID).
%
Once again, only one thread will be able to atomically update $shadow[0]$, at which point all other threads will find the new \textbf{GLOBAL READ} state and will proceed to recalculate the next state.
%
Since there is no further classification of reads, all remaining threads executing this instruction and finding $shadow[0]$ in the \textbf{GLOBAL READ} state will leave the state unchanged.

Concurrently, threads will be executing line 6 to write values to various indices within the $data$ array. Thread 2, for example, will write to $data[1]$, finding $shadow[1]$ to still be in the \textbf{INIT} state. It will then update $shadow[1]$ to the \textbf{WRITE} state.
%
At some point, thread 1 will attempt to write to $data[0]$ and may find it in one of two possible states:

\begin{enumerate}
    \item \textbf{READ} state with its own ID if no other accessor has completed its read / update, or 
    \item \textbf{GLOBAL READ} state (with any ID) if multiple accessors have read $data[0]$.
\end{enumerate}

In the first case, since the same thread is writing it will update $shadow[0]$ to the \textbf{WRITE} state. From this state, the next thread to complete the read access on line 4 will find $shadow[0]$ in the \textbf{WRITE} state with a different thread ID, and follow the \textbf{$\text{R}_\text{G}$} edge to indicate a race.
%
In the second case, thread 1 will follow the \textbf{$\text{W}_\text{*}$} edge from \textbf{GLOBAL READ} to indicate a race (* indicates any thread relation to the prior accessor, including itself).
%
At this point, a race will be called out, and all future accesses to $data[0]$ will find $shadow[0]$ in the \textbf{RACE} state and cease updating the shadow value.

% ---------------

\begin{figure}[]
    %\centering
    \includegraphics[width=0.5\textwidth]{figures/ssm_blocksync.png}
    \caption{State-Machine with Block Synchronization (self loops omitted)}
    \label{fig:ssm_bsync}
\end{figure}


\input{figures/code_rwrace_bsync}

To take the design intuition one step further, we expand the set of programs to include those just discussed as well as programs that include thread-block synchronization, such as in Listing~\ref{lst:rw-bsync}.

We can immediately see a flaw in our 5-state state-machine; if all threads are members of the same thread-block, then the write on line 7 is not concurrent with any reads on line 4, but our state-machine will step into the \textbf{RACE} state.
%
To handle this added complexity, we expand the state-machine to that shown in Figure~\ref{fig:ssm_bsync}.

An important observation is that this expanded state machine is a super-set of the original, smaller machine. The same states are present, and all unsynchronized accesses either from the same thread, or between threads sharing only the global scope (i.e. not within a shared thread-block) follow the same transitions between the original states.
%
As such, we need only focus our attention on the newly introduced elements. 

Focusing on~\ref{lst:rw-bsync}, we return to the state of $shadow[0]$ once a single thread has executed line 4, leaving it in the \textbf{READ} state. 
%
We are left with a different set of possibilities here:
\begin{enumerate}
    \item The kernel is executed with only a single thread-block, or
    \item The kernel is executed with multiple thread-blocks.
\end{enumerate}

If all threads are members of a single thread-block, then no threads may proceed past line 5 until all have completed the read access, leaving $shadow[0]$ in the \textbf{BLOCK READ} state. 
%
At this point each thread participating in the \emph{\_\_syncthreads()} will increment a local scalar clock, and execution will proceed to line 7.
%
(Note that no memory access occurs on line 5, so there are no state changes until the next memory access.)
%
When thread 1 accesses $data[0]$, it will find $shadow[0]$ in the \textbf{BLOCK READ} state; however, it will also find a scalar clock value of 0, which when compared against it's local clock value of 1 indicates that the current access follows a block synchronization point, so that it will follow either the \textbf{$\text{W}_\text{\{Bs, S\}}$} or \textbf{$\text{W}_\text{\{Bs, B\}}$} transition (depending on the prior accessor) and transition safely to the \textbf{WRITE} state.

For the second case (multiple thread-blocks) the same set of transitions is possible if one thread-block executes to completion prior to any other executing.
%
In that situation, all threads from the second thread-block share only the global scope with all prior accessors, and thus the \textbf{$\text{R}_\text{\{*, G\}}$} transition will result in $shadow[0]$ transitioning to the \textbf{RACE} state with the first update.
%
Notably, although threads from separate thread-blocks will compare their scalar clocks, since the clock represents a thread-block level event it has no effect on the transitions for global-scope threads.

However, when a separate thread-block executes concurrently we may find that the read access on line 4 between threads sharing only a global scope will leave $shadow[0]$ in the \textbf{GLOBAL READ} state.
%
From this state, without support for synchronization across the global scope, any write will transition to the \textbf{RACE} state. 

The result is that when only a single thread-block is spawned, the kernel shown in Listing~\ref{lst:rw-bsync} does not contain a date race, and our state machine has no path to the \textbf{RACE} state regardless of the number of threads within the thread-block.
%
On the other hand, when 2 or more thread-blocks are spawned all possible thread schedules will inevitably lead to the \textbf{RACE} state.


\begin{figure}[]
    %\centering
    \includegraphics[width=0.5\textwidth]{figures/shadow_mem.png}
    \caption{Shadow memory}
    \label{fig:ssm_shadow}
\end{figure}




% \hspace{2in}
% \hrulefill
% \hspace{2in}


% \input{figures/code_rwrace_nosync}

% \ggcmt{One shadow item is tracked in HiRace (R or W). Our SM can go by this to check races.}

% \ggcmt{iGuard and other tools and TSan  keep   N (=2, or =4) access records. Due to conflicts if gets discarded, we miss races.}

% Table/comparisons are the guiding principle to code in other checkers.

% \ggcmt{For us, an explicit state machine has these advantages: encapsulates info in a modular way plus Murphi formal checking.}

% \ggcmt{Here, a short example will help explain the ensuing material--walk-through of the algo, state-machine, and Fig-1. Thru 2-3 iterations, we will show how the algo's parts add up.}

% By way of example, consider the code in Listing~\ref{lst:rw-nosync}. Prior to any memory access, all accesses are legal so we initialize all shadow values to an Initial state. Regardless of access order, the first thread to update the shadow value for this memory will record its own ID and a single read access. 

% Traditional vector clocks are generally infeasible for GPU's due to their poor scaling with thread counts, but it is sufficient in this case to use a scoped scalar clock inspired by other recent works (\cite{fasttrack}, \cite{iguard}). We instrument each synchronization point in the program to maintain a clock for the entire scope of that synchronization, and each thread tracks the latest clock for the widest scope synchronization seen since its last access. In the case of non-hierarchical scopes (i.e. multiple overlapping sub-warp masked synchronization, with non-empty symmetric difference) more fine-grained clocks must be maintained; once such a case is detected \toolname begins storing a temporary indexed history of all non-hierarchical scoped synchronizations until a fully encompassing sync point supersedes it, at which point the history may be discarded. This approach could become prohibitively expensive as in the extreme case this approach devolves to essentially a full vector clock tracking individual thread interactions, but we find that this uncommon in practice and provide flags to enable or disable the tracking of these fine-grained interactions to avoid excess memory usage in the general case.

% To provide flexibility and improved performance to users \toolname allows custom configurations of its metadata structure and the usage of less common features, as well as the ability to track only user-specified data sets. Expensive features such as fine-grained thread interaction tracking must be enabled to allocate additional memory to tracking non-hierarchical synchronizations, but when disabled the user may opt for either a conservative approach which ignores these synchronization points entirely and thus introduces additional false positives, or alternatively may suppress races that fall within these regions. To further retain performance for practical usage, we require manual user annotation for lock and release/acquire pattern recognition. We find that overhead of automatic inference of these patterns is prohibitively expensive, and also that these patterns aren't generally practical for higher performance GPU code.

% Utilizing these methods, \toolname by default uses only 8 bytes of memory per data address by default, and is configurable to use less when possible.

% Each transition in the SSM is determined by a product of three relations between the prior and current accesses; the current access type, synchronization scope, and thread relation. Access type refers to the specific memory action and includes reads, writes, and atomic accesses. Synchronization scope captures the happens-before relation between accesses and reduces it to binary scope-level synchronization status (i.e. synchronized or un-synchronized access at a particular scope.) Thread relation captures the smallest shared scope of the prior and current accessing threads.

% By way of example, consider a system with no memory ordering primitives (i.e. no synchronization) or atomics. The SSM shown in Fig. \ref{fig:ssm_nosync} is sufficient to capture all shared memory interactions in such a system. With no synchronization we only need consider whether two threads are the same or not, so the smallest shared scope between any two distinct threads is global. With only reads and writes and two thread relations, each state only has 4 transitions. 

% From an initial un-accessed state we have no past accessor to compare against, so we simply record the first read or write to this memory location along with the accessing threads ID. 


% \hspace{2in}

% components:
% \begin{itemize}
%     \item memory access ordering
%     \item memory access activity/history (read/write)
%     \item access safety scope
% \end{itemize}



% Our design is based on tracking an "access safety" property for each memory location. 


% \begin{itemize}
%     \item build up from intuition:
%     \item introduce simple monotonic safety design with no back edges (no sync.)... maybe initially with CPU in mind?
%     \item optimize with internal state-machine abstraction
%     \item fit to CUDA / GPU design if not yet introduced; thread / mem hierarchies and their impact on state-machine
%     \item sub-warp analysis
%     \item ---
%     \item abstractions:
%     \item "access safety" property
%     \item internal state-machine
%     \item last accessor
%     \item AP regions (LD Terminology)
%     \item ---
%     \item impl method:
%     \item template library
%     \item config params
% \end{itemize}

% strategy for developing logical components:
% \begin{enumerate}
%     \item consider, for a single memory address, a relevant memory interaction (i.e. a load, a store, atomic access, whatever) in the absence of synchronization primitives like sync, fences, etc.
%     \item from initial un-accessed memory state, any access by any thread is legal.
%     \item after this interaction, what other interactions are legal? create state for each such interaction, continuing until looping in race state. with no sync considerations, should be able to form a DAG from initial state to race
%     \item now consider synchronization effects and add appropriate back edges. at this point, scoped synchronization primitives become relevant so determine if additional state is needed to record history, particularly hierchically nested scope history (i.e. multiple reads within a warp, following a properly scoped warp synchronization, following block sync'd reads, which follow a block scope write.) 
% \end{enumerate}

% atomic handling:
% \begin{itemize}
%     \item atomics are basically loads, so a single "naked" atomic access is basically in the write state (but needs to be separate for atomic identifier)
%     \item global atomic: a write that is only naturally synchronized with other global atomics, or block atomics within the same block
%     \item need to track historical reads to determine safety of more narrow atomics / sync
%     \item so should consider:
%         1) single glob. atomic, 
%         2) grid scope accesses between glob. atomics, can never be safe to access again except by global atomics, 
%         3) block scope accesses by glob atomics, safe for block atomic access (transition to 2 below), can be sync'd by block scope syncs 
%         4) warp scope accesses by glob atomics, safe for block atomic access, can be sync'd by block or appropriate warp syncs
%     \item block atomic: only safe for atomic access within the block
%         1) single block atomic
%         2) block scope atomic accesses, 
% \end{itemize}





% tracking minimal metadata per memory location. To achieve this, we first represent hierarchical thread groups as single accessor entities to reduce the overhead of tracking individual threads. This allows us to further reduce the access history representation we achieve a more compact state that exhaustively

% we enumerate arbitrary access history patterns and reduce them to equivalence classes. By further equating hierarchical thread groups as accessor entities to reduce the overhead of tracking individual threads, we achieve a more compact state that exhaustively.


% Single-accessor checking is made possible by our novel finite state machine which compactly encodes . Our FSM supplements the prior accessors metadata with minimal historical access metadata, most notably a summarized access history and the shared scope of all accessors. This enhancement is especially influential in a hierarchical work group setting as it enables us to represent the access history of large groups of accessing threads as a single unit.

% \begin{compactitem}
% \item Walk-thru simple code example
% \item One line accomplishes a ``ripple-effect'' of checks at many levels of the hierarchy
% \item Then a sync comes in, calling for a fleshed-out version of the SM
% \end{compactitem}

==> sections/eval.tex <==

\subsection{Experimentation Methodology}

Our experiments were executed on a system with the following configuration:

\begin{itemize}
    \item CPU: AMD Ryzen 5 3600
    \item GPU: NVIDIA Geforce RTX 2070 Super
    \item OS: Ubuntu 22.04
    \item CUDA version: 11.7
\end{itemize}


\subsection{Section: Indigo Benchmarks}
%\ggcmt{mb describes the "calibrated benchmark generator" here}
We use programs and inputs from the recently released Indigo benchmark suite~\cite{mb-ispass22} to drive our experiments. Unlike conventional suites, Indigo contains scripts and configuration files that allow the user to generate the desired codes and inputs. 

There are 14 graph generators to choose from for creating parameterizable inputs of arbitrary size. There are also 21 CUDA kernel generator patterns which generate up to 580 distinct CUDA programs operating on a given input data type.

More importantly for us, the code generator is not only able to synthesize hundreds of different versions of common graph-processing code patterns but also to systematically insert various bugs. We make extensive use of this latter capability as it enables us to control precisely which bugs, if any, are present. This provides a reliable ground truth valuation, which is typically not available with other suites or codes. 
%
Each benchmark kernel comes paired with a sequential implementation of the same algorithm as a baseline verification of the benchmarks correctness (or lack thereof.)

%\mbcmt{maybe mention how many CUDA codes in total, how many buggy codes, and how many inputs were generated and used}

\subsection{Results}

%o\ggcmt{JJ will describe Table 2 roughly here. Also Fig4 might be replaced by a table/?}

For our tests we used Indigo to generate 580 CUDA kernels, of which 346 contained data races. We also generated a number of small input graphs for testing the accuracy of \toolname{}, and used 6 graphs ranging between 5 nodes and 200 nodes to evaluate both \toolname{} and \iguard; the results are displayed in Table~\ref{tab:errors-found}.

We also compared our results to cuda-memcheck, but since it only checks for shared memory races there were relatively very few examples to compare against, and both \iguard and \toolname{} seemed to perform on par with cuda-memcheck when relevant.

We found that on the 3480 Indigo benchmark comparisons between \iguard and \toolname{}, neither tool provided any false positives. While \iguard performed quite well in identifying data races given the constraints of classical race detection algorithms, \toolname{} was able to find 100\% of the injected data races in the Indigo benchmarks (when provided with inputs that exhibited the injected data race.)

Further, we tested the same codes on eleven large scale real-world graph inputs (as described in Table~\ref{tab:large-graphs}) to test performance, as shown in Figure~\ref{fig:speedup_iguard}.
%
\iguard struggled with very large grid dimensions, and the timing results were very sporadic (occasionally requiring multiple hours at thousands of times slowdown from baseline code execution.)
%
We were able to compare 441 executions across these large graphs to \iguard, which demonstrated an overall average overhead of more than 30x slowdown, against \toolname{}'s average of less than 3x slowdown across the same set of test code / input combinations.

With \toolname{}'s low overhead we were able to more thoroughly test its performance against baseline codes. Across 5,105 executions (464 Indigo codes across the 11 large graphs in Table~\ref{tab:large-graphs}) \toolname{} demonstrated 7.5x average slowdown, and 1.08x median slowdown (while still identifying 100\% of injected data races, with no false positives!)

\toolname{} also had a small number of outliers, primarily due to its race reporting scheme which required significantly more I/O on some code patterns to report races on unique memory addresses.

Lastly, using our default shadow value footprint of 8 bytes per tracked memory address, we operate at less than half of the memory overhead of \iguard. In real application we would be able to reduce this footprint further by configuring \toolname{}'s settings to more efficiently track the parallel patterns in a given test application.



\input{figures/table_large_graphs}


\input{figures/table_correctness}


\begin{figure}[]
    %\centering
    \includegraphics[width=\linewidth]{figures/speedup_vs_iguard.png}
    \caption{HiRace speedup vs. iGuard. Each point represents execution of one Indigo benchmark kernel on the associated input graph.}
    \label{fig:speedup_iguard}
\end{figure}

% Implementing as template library and manual instrumentation on:
% \begin{itemize}
%     \item indigo - need to test on different input sizes, ensure determinism, and run with different kernel params (thread / block distribution)
%     \item need to test config optimizations (reducing monitored tid/bids, reducing region counter storage, testing variable subsets, ...) for performance gains and retained accuracy
%     \item comparing at least iguard, and can compare cuda-racecheck for shared memory examples?
%     \item Martin TSP codes
%     \item other good test examples above "toy scale"?
%     \item need "real scale" regular code for perf. tests... any suggestions?
% \end{itemize}

% \subsection{Discussions}
% \ggcmt{Good not to just list results one after the other; at least have a few assessment bullets, recaping what was achieved.}
% \begin{itemize}
% \item key takeaways
% \item from this work
% \end{itemize}


==> sections/extable2.tex <==
\begin{center}
\begin{tabular}{|c|c|ll|c|c|}
\cline{1-2} \cline{5-6}
\multicolumn{1}{|c|}{$x$} & \multicolumn{1}{c|}{$\Phi^+(x)$} &  &  & \multicolumn{1}{c|}{$x$} & \multicolumn{1}{c|}{$(\Phi^+)'(x)$} \\ \cline{1-2} \cline{5-6} 
-0.000                     & 1.000                         &  &  & -0.000                    & 0.100                            \\
-0.100                     & 0.110                         &  &  & -0.100                    & 0.011                            \\
-1.000                     & 0.100                         &  &  & -1.000                    & 0.010                            \\
-1.100                     & 0.011                         &  &  & -1.100                    & 0.010                            \\ \cline{1-2} \cline{5-6} 
\end{tabular}
\captionof{table}{Illustration of LNS via an example. First, two tables, the left-hand one for computing $\Phi^+(x)$ and the right-hand one for performing first-order interpolation as per Equation~\ref{eq:T} are created and employed as described in Section~\ref{sec:pd}.}
\label{tab:lns-illustration}
\end{center}

==> sections/impl.tex <==

% \ggcmt{JJ: Engineering details - Elaboration of SEc3 wrt impl details}

\toolname{} is implemented primarily as a template library, alongside Clang's AST tools for automated instrumentation. Its configuration is exposed through a \emph{toml} interface, allowing the user to specify a number of features, such as which kernels and variables to monitor for races, thread groups to monitor, and bounds for shadow value metadata to reduce memory overhead.


%%
\subsection{Race Detection Algorithm}
\input{figures/pseudocode_shadow_update}

The core of HiRace race detection is the shadow state update algorithm (Algorithm~\ref{algo:updateShadow}) built around the state machine described in Section~\ref{sec:design}.

Our currently implemented state machine contains 25 states and 1200 transitions, requiring only 5 bits of memory per monitored memory address, as opposed to 42 bits needed to uniquely identify an additional prior accessor in iGuard.
%
\toolname supports:
\begin{enumerate}
    \item Three thread hierarchies (i.e. thread-block, warp, and inter-warp thread scopes.)
    \item Synchronization primitives for each  hierarchy.
    \item Atomic memory accesses.
\end{enumerate}
%
We have also verified this version of the state machine with an exhaustive state space search in Murphi, demonstrating that arbitrary access patterns (within the supported set of operations) correspond accurately to race or non-race states.

The \emph{UpdateShadow} function is called at each memory access by the accessing thread to compare the prior access metadata to current access metadata.
%
Another benefit of our state machine design is that race detection logic is baked into the state machine itself. As a result, the only computation needed to detect races at runtime are to determine the relationship between the current and prior accessing thread, and the synchronization relationship based on scalar clock values.
%
Our state machine is realized as a map from transition ID's to states, and is encoded as a  flat array, ordered by the transition elements (i.e. prior state, memory action, sync relation, and thread relation.) 
%
After computing the aforementioned relations, the resulting values are combined into an index into the state machine array.

This update logic is implemented in a lock-free loop to ensure system progress.



%%
\subsection{Memory Access Monitoring}

To capture memory accesses \toolname utilizes a templated wrapper class to track user data pointers and their associated shadow value pointers.
%
Each monitored variable is tracked within a thread local wrapper which overrides standard operators to intercept memory access events and update the associated shadow value transparently.

This approach allows flexible management of the underlying test data structures, as well as their associated shadow structures and thread metadata.
%
Individual threads or test data addresses may have their instrumentation enabled or disabled dynamically, and memory footprint may be reduced by tracking only representative threads for user defined symmetric work groups instead of tracking all threads.

This approach also requires overriding other relevant functions, such as atomic functions. This is easily achieved by overloading the relevant functions for calls on our pointer wrapper class.


%%
\subsection{Source Instrumentation}

Lastly, to facilitate instrumentation of our wrappers we provide a standalone Clang tool for AST parsing and rewriting. 

The Clang LibTooling C++ interface facilitates parsing source code into AST, as well as walking the AST and rewriting the AST and/or source code through a robust API.
%
It allows us to identify elements of the test code to be monitored and properly alias shared memory pointers through our wrapper class, as well as allocate necessary memory for shadow value tracking.












% \begin{itemize}
%     \item Expt methodology, machines, instr methods,

%     \item Eval case studies:

%     \begin{itemize}
%         \item Irreg codes studied: gen nature

%         \item reg codes 
        
%     \end{itemize}

% \item Tools we compare against: iGuard, CUDA memcheck

%  \begin{itemize}
%      \item how we bettered over iGuard in terms of litmus tests. Informs of the possibility of adaptations we will make.

% \item ThreadFence wrong in iGuard and how we handle it

% \item iGuard overheads due to Jitting
     
%  \end{itemize}
 
% \item Kinds of measurements we will do, parameters of the examples that are relevant to race checking (threads, blocks,...) that we will vary


    
% \end{itemize}

% {\em .75 pages into IMPL}


% To avoid data movement and communication with the host machine, race detection is takes place entirely on the GPU. This allows us to utilize resources and patterns employed in the test code for a natural parallel implementation with each thread logging its own access histories. To achieve this, \toolname is implemented as a Clang source rewriting front end along with a header library containing the safety state machine description and necessary metadata analysis functions.

==> sections/misc.tex <==
\begin{itemize}
    \item \textbf{TODO: Sanitize for double-blind review!}
    \item Supercomputing info: \url{https://sc23.supercomputing.org/program/papers/}
    \item Submission deadline: Abstract 03/30, full 04/06
    \item Maximum 10 pages (excl. bib)
    \item reproducibility/artifacts important
\end{itemize}


some meeting notes:
martin paper ideas:
1. first just explain simple state machine (maybe single block with syncthreads.)
2. now explain in text only how to extend to support multi block, then others, etc.
3. then describe verification with model checker
4. maybe demo this process against the simple model (like show a simple murphi model tested against the simpler state machine.)
5. then jsut say full model will be released with code.

main thing is to translate the key idea.

one approach is to tackle the problems reviewers might have with verification specifically... i.e. can we prove explicitly that the data we track is enough.

be sure to explicitly state all verified assertions / properties

martins paper writing :

1. outline
2. intro
3. then explain approach in detail
4. related works
5. methodology / exper.
6. results
7. then abstract / conclusions

paper is not a description of your research, but teaching people how to repeat what you did
